A General Probabilistic Approach for Quantitative Assessment of LES Combustion Models

The Wasserstein metric is introduced as a probabilistic method to enable quantitative evaluations of LES combustion models. The Wasserstein metric can directly be evaluated from scatter data or statistical results using probabilistic reconstruction against experimental data. The method is derived and generalized for turbulent reacting flows, and applied to validation tests involving the Sydney piloted jet flame. It is shown that the Wasserstein metric is an effective validation tool that extends to multiple scalar quantities, providing an objective and quantitative evaluation of model deficiencies and boundary conditions on the simulation accuracy. Several test cases are considered, beginning with a comparison of mixture-fraction results, and the subsequent extension to reactive scalars, including temperature and species mass fractions of \ce{CO} and \ce{CO2}. To demonstrate the versatility of the proposed method in application to multiple datasets, the Wasserstein metric is applied to a series of different simulations that were contributed to the TNF-workshop. Analysis of the results allowed to identify competing contributions to model deviations, arising from uncertainties in the boundary conditions and model deficiencies. These applications demonstrate that the Wasserstein metric constitutes an easily applicable mathematical tool that reduce multiscalar combustion data and large datasets into a scalar-valued quantitative measure.

==> Append.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\appendix
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\label{APP_WM_GEN_PROB_MEASURE}Wasserstein metric for general probability measures}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
Let $(M,\, d)$ denote a complete separable metric space equipped with distance functions $d$, on which there are two probability measure $\mu$ and $\nu$ with finite $p^{\text{th}}$ moments. Following Kantorovich's formulation, we have the $p^{\text{th}}$ Wasserstein metric between $\mu$ and $\nu$ defined as
\begin{equation}
\label{eq_general_wasserstein_metric}
	W_p(\mu,\,\nu) = \bigg( \inf_{\gamma \in \Gamma(\mu,\,\nu) } \int_{M \times M} d(x,\,y)^p \, d\gamma(x,\,y) \bigg)^{1/p},\,
\end{equation}
where $ \Gamma(\mu,\,\nu) $ is a set of admissible measures $\gamma$ on $M \times M$, whose marginals are $\mu$ and $\nu$.

Specifically for continuous distributions defined on the Euclidean space with $M = \mathbf{R}^d$ and $d(x,\,y) = |x-y|$, the measures $\mu$ and $\nu$ can be represented by their probability density functions denoted by $f$ and $g$. Thus, we can rewrite the definition in Eq.\ref{eq_general_wasserstein_metric} as
\begin{equation}
\label{eq_euclidiean_wasserstein_metric}
	W_p(\mu,\,\nu) = \bigg( \inf_{h \in G(f,\,g)} \int_{\mathbf{R}^d} \int_{\mathbf{R}^d} d(x,\,y)^p h(x,\,y) \, dx \, dy \bigg)^{1/p},\,
\end{equation}
where $G(f,\,g)$ is a set of joint probability density functions, whose marginal density functions satisfy
\begin{align}
	\int_{\mathbf{R}^d} h(x,\,y) \, dy &= f(x) \, ,\\
	\int_{\mathbf{R}^d} h(x,\,y) \, dx &= g(y)\,.
\end{align}

The formulation in Eq.~\ref{eq_euclidiean_wasserstein_metric} of the Wasserstein metric entails two different interpretations. The first interpretation is very close to the origin of the optimal transportation problem. If each distribution is viewed as a pile of ``dirt" distributed in the Euclidean space according to the probability, the metric is the minimum amount of work required to turn one pile into the other. The transport plan $h(x,\, y)$ represent the density of mass to be transported from $x$ to $y$. The second interpretation views $h(x,\, y)$ as the joint distribution of $x$ and $y$ whose marginal distributions match $f$ and $g$.  The Wasserstein metric is the minimal expectation of the distance between $x$ and $y$ among all such distributions. 

For the special case of one-dimensional distributions on the real line, the Wasserstein metric possesses many useful properties~\cite{bobkov2014one, Cohen1997}. Let $F$ and $G$ be the cumulative distribution functions for one-dimensional distributions $\mu$ and $\nu$, while $F^{-1}$ and $G^{-1}$ being their corresponding inversions. The Wasserstein metric can then be written in the explicit form as
\begin{equation}
\label{eq:w_p_cdf}
	W_p(\mu,\, \nu) = \bigg(\int_{0}^{1} | F^{-1}(x) - G^{-1}(x) |^p dx \bigg)^{1/p}\,.
\end{equation}
Furthermore, when $\mu$ and $\nu$ are 1D empirical distributions with the same number of samples, the relationship in Eq.~\ref{eq:w_p_cdf} can be further simplified as 
\begin{equation}
\label{eq:w_p_edf}
	W_p(\mu,\, \nu) = \bigg( \frac{1}{n} \sum_i^n |x_i^* - y_i^*|^p \bigg)^{1/p}\,,
\end{equation}
where $x^*_i$ and $y^*_i$ are $x_i$ and $y_i$ in sorted order. 


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{\label{APP_SRC_CODE}Sample code for the evaluation of the multidimensional Wasserstein metric}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Sample code is provided for three Wasserstein metric cases: one-dimensional (Z), two-dimensional (Z-T), and four-dimensional (Z-T-CO2-CO). The code, available at \comment{TBD: publicly-accessible html}, is easily adaptable for additional trial cases. The implementation of the sample code mirrors the procedure laid out in Section~\ref{SSEC_CALC_PROC}. \textit{sampleWasserstein.m} serves as the main script, while \textit{calcW2.m} is the function that calculates the Wasserstein metric.

Inputs to \textit{calcW2.m} include experimental and simulated data samples for the Sydney piloted jet flame, at $x/D_J = 10$, $r/D_J =0.6$, as well as a list of comparison species. Outputs include the calculated Wasserstein metric ($W_2$), flow matrix, and data visualizations (for one-dimensional and two-dimensional cases, only). Additional cases can be calculated by modifying the \textit{species\_index} input, where the available species include Z, T, $Y_{\ce{CO_{2}}}$, and $Y_{\ce{CO}}$.


==> abbrevs.tex <==
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\makeatletter
\newcommand\rlarrows{\mathop{\operator@font \rightleftarrows}\nolimits}
\makeatother
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\newenvironment{itemizePacked}{
\begin{itemize}
  \setlength{\itemsep}{1pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{itemize}}
\newenvironment{enumeratePacked}{
\begin{enumerate}
  \setlength{\itemsep}{5pt}
  \setlength{\parskip}{0pt}
  \setlength{\parsep}{0pt}
}{\end{enumerate}}
% abbreviations %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\def\codefont{scriptsize}
\newcommand{\f}[2]{{\frac{#1}{#2}}}
\newcommand{\wt}[1]{{\widetilde{#1}}}
\newcommand{\wh}[1]{{\widehat{#1}}}
\newcommand{\wc}[1]{{\widecheck{#1}}}
\newcommand{\chem}[1]{\ensuremath{\mathrm{#1}}}
\newcommand{\lrangle}[1]{{\langle{#1}\rangle}}
%\newcommand{\lrangle}[1]{{\left\langle{#1}\right\rangle}}
\newcommand{\lrcurl}[1]{{\{{#1}\}}}
%\newcommand{\lrcurl}[1]{{\left\{{#1}\right\}}}
\newcommand{\ol}[1]{{\overline{#1}}}
\newcommand{\ul}[1]{{\underline{#1}}}
\newcommand{\tr}{{\scriptscriptstyle\mathsf T}}
\newcommand{\dd}{{\scriptscriptstyle\Delta}}
\newcommand{\suble}{{\scriptscriptstyle <}}
\newcommand{\eps}{{\varepsilon}}
\def\REFUP{\rm{ref}}
\def\REF{_{\REFUP}}
\def\RPP{reaction progress parameter}

% boldface-italic font
\newcommand{\bfit}[1]{\textbf{\textit{#1}}}

%
% SOME COLORS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\newcommand{\colred}[1]{{\color{red} #1}}
\newcommand{\colblue}[1]{{\color{blue} #1}}
\newcommand{\colwhite}[1]{{\color{white} #1}}
\newcommand{\colgreen}[1]{{\color{green} #1}}
\newcommand{\colbrown}[1]{{\color{Brown} #1}}
\newcommand{\colfucsia}[1]{{\color{Fuchsia} #1}}
\newcommand{\colBlue}[1]{{\color{Blue} #1}}
\newcommand{\corrections}[1]{{\color{blue}\it#1}}
%
% FOR COMBUSTION TEXT %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\chist{\chi_{Z,\up{st}}}
\def\chiq{\chi_{Z,\up{q}}}
\def\chii{\chi_{Z,\up{i}}}
%
% Standard TEX-abbreviations used %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\cldbpage{\clearpage{\pagestyle{empty}\cleardoublepage}}
%
% CALIGRAPHICAL SYMBOLS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\cA{{\cal{A}}}
\def\cB{{\cal{B}}}
\def\cC{{\cal{C}}}
\def\cO{{\cal{O}}}
\def\cD{{\cal{D}}}
\def\cE{{\cal{E}}}
\def\cF{{\cal{F}}}
\def\cH{{\cal{H}}}     % Heaviside function
\def\cG{{\cal{G}}}     % LES transfer function
\def\cN{{\cal{N}}}     % New variable
\def\cM{{\cal{M}}} 
\def\cL{{\cal{L}}}     % Size of domain
\def\cS{{\cal{S}}}     % norm of strain rate tensor
\def\cT{{\cal{T}}}
\def\cU{{\cal{U}}}
\def\cC{{\cal{C}}}     %
\def\cM{{\cal{M}}}     %
\def\cP{{\cal{P}}}     %
\def\cR{{\cal{R}}}     %
\def\cV{{\cal{V}}}     %
\def\cQ{{\cal{Q}}}     %
%
% NEW FUNCTION NAMES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\erf{{\rm{erf}}}
%
% TEXT FONT DEFINITIONS %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\up{\textup}
\def\p{\partial}
\def\d{\textup d}
\def\D{\displaystyle}
%\def\S{\scriptsize}
\def\OmFint{\iiint\limits_{\OmF}}
\def\OmF{{\Omega_{\cal F}}}
\def\OmA{{\Omega_{\cal A}}}
\def\e{\textup{e}}
\def\i{\textup{i}}
%
% DIMENSIONLESS QUANTITIES %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
%\def\Re{{\rm{Re}}}
\def\Fr{{\rm{Fr}}}
\def\M{{\rm{M}}}
\def\Re{{\rm{Re}}}
\def\Rd{{\rm{Rd}}}
\def\Le{{\rm{Le}}}
\def\Da{{\rm{Da}}}
\def\Ka{{\rm{Ka}}}
\def\Nu{{\rm{Nu}}}
\def\Sc{{\rm{Sc}}}
\def\Ri{{\rm{Ri}}}
\def\Ec{{\rm{Ec}}}
\def\Tu{{\rm{Tu}}}
\def\St{{\rm{St}}}
\def\Mi{{\rm{Mi}}}
\def\Ra{{\rm{Ra}}}
%
% FOR LATEX %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
 \def\avec{{\mbox{\boldmath$a$}}}
 \def\bvec{{\mbox{\boldmath$b$}}}
 \def\Bvec{{\mbox{\boldmath$B$}}}
 \def\cvec{{\mbox{\boldmath$c$}}}
 \def\dvec{{\mbox{\boldmath$d$}}}
 \def\evec{{\mbox{\boldmath$e$}}}
 \def\Fvec{{\mbox{\boldmath$F$}}}
 \def\Nvec{{\mbox{\boldmath$N$}}}
 \def\fvec{{\mbox{\boldmath$f$}}}
 \def\gvec{{\mbox{\boldmath$g$}}}
 \def\hvec{{\mbox{\boldmath$h$}}}
 \def\ivec{{\mbox{\boldmath$i$}}}
 \def\jvec{{\mbox{\boldmath$j$}}}
 \def\kvec{{\mbox{\boldmath$k$}}}
 \def\pvec{{\mbox{\boldmath$p$}}}
 \def\Pvec{{\mbox{\boldmath$P$}}}
 \def\uvec{{\mbox{\boldmath$u$}}}
 \def\Uvec{{\mbox{\boldmath$U$}}}
 \def\nvec{{\mbox{\boldmath$n$}}}
 \def\tvec{{\mbox{\boldmath$t$}}}
 \def\Rvec{{\mbox{\boldmath$R$}}}
 \def\rvec{{\mbox{\boldmath$r$}}}
 \def\svec{{\mbox{\boldmath$s$}}}
 \def\Svec{{\mbox{\boldmath$S$}}}
 \def\xvec{{\mbox{\boldmath$x$}}}
 \def\vvec{{\mbox{\boldmath$v$}}}
 \def\wvec{{\mbox{\boldmath$w$}}}
 \def\yvec{{\mbox{\boldmath$y$}}}
 \def\mvec{{\mbox{\boldmath$m$}}}
 \def\Xvec{{\mbox{\boldmath$X$}}}
 \def\qvec{{\mbox{\boldmath$q$}}}
 \def\0vec{{\mbox{\boldmath$0$}}}
 \def\xivec{{\mbox{\boldmath$\xi$}}}
 \def\rhovec{{\mbox{\boldmath$\rho$}}}
 \def\wpvec{{\boldsymbol{\wp}}}
 \def\psivec{{\mbox{\boldmath$\psi$}}}
 \def\epsvec{{\mbox{\boldmath$\epsilon$}}}
 \def\phivec{{\mbox{\boldmath$\phi$}}}
 \def\varphivec{{\mbox{\boldmath$\varphi$}}}
 \def\zetavec{{\mbox{\boldmath$\zeta$}}}
 \def\kappavec{{\mbox{\boldmath$\kappa$}}}
 \def\varkappavec{{\pmb{\varkappa}}}
 \def\etavec{{\mbox{\boldmath$\eta$}}}
 \def\Psivec{{\boldsymbol{\Psi}}}
 \def\Phivec{{\boldsymbol{\Phi}}}
 \def\Wvec{{\boldsymbol{W}}}
 \def\Yvec{{\mbox{\boldmath$Y$}}}
 \def\Vvec{{\mbox{\boldmath$V$}}}
 \def\cLvec{{\boldsymbol{\cal{L}}}}
 \def\cMvec{{\boldsymbol{\cal{M}}}}
 \def\omegavec{{\mbox{\boldmath$\omega$}}}
 \def\Omegavec{{\mbox{\boldmath$\Omega$}}}
 \def\sigmavec{{\boldsymbol{\sigma}}}
 \def\Amat{{\underline{\underline{{A}}}}}
 \def\Bmat{{\underline{\underline{{B}}}}}
 \def\Phimat{{\underline{\underline{{\Phi}}}}}
 \def\taumat{{\underline{\underline{{\tau}}}}}
 \def\sigmamat{{\underline{\underline{{\sigma}}}}}
 \def\Cmat{{\underline{\underline{{C}}}}}
 \def\Imat{{\underline{\underline{{I}}}}}
 \def\Jmat{{\underline{\underline{{J}}}}}
 \def\Smat{{\underline{\underline{{S}}}}}
 \def\Rmat{{\underline{\underline{{R}}}}}
 \def\Tmat{{\underline{\underline{{T}}}}}
 \def\Emat{{\underline{\underline{{E}}}}}
 \def\tmat{{\underline{\underline{{t}}}}}

 \def\alphavec{{\boldsymbol{\alpha}}}
 \def\betavec{{\boldsymbol{\beta}}}
 \def\tauvec{{\boldsymbol{\tau}}}
 \def\thetavec{{\boldsymbol{\theta}}}
 \def\lambdavec{{\mbox{\boldmath$\lambda$}}}
 \def\cTmat{{\underline{\underline{{\cal{T}}}}}}
 \def\cLmat{{\underline{\underline{{\cal{L}}}}}}
 \def\cMmat{{\underline{\underline{{\cal{M}}}}}}
 \def\kappamat{{\underline{\underline{{\kappa}}}}}
%
% Grad, Div, ... %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%
\def\Grad{\nabla}
\def\Div{\nabla \cdot}
\def\Lap{\nabla^2}
%

